Randomized Iterative Algorithms for Fisher Discriminant Analysis

Fisher discriminant analysis (FDA) is a widely used method for classification and dimensionality reduction. When the number of predictor variables greatly exceeds the number of observations, one of the alternatives for conventional FDA is regularized Fisher discriminant analysis (RFDA). In this paper, we present a simple, iterative, sketching-based algorithm for RFDA that comes with provable accuracy guarantees when compared to the conventional approach. Our analysis builds upon two simple structural results that boil down to randomized matrix multiplication, a fundamental and well-understood primitive of randomized linear algebra. We analyze the behavior of RFDA when the ridge leverage and the standard leverage scores are used to select predictor variables and we prove that accurate approximations can be achieved by a sample whose size depends on the effective degrees of freedom of the RFDA problem. Our results yield significant improvements over existing approaches and our empirical evaluations support our theoretical analyses.

==> Definitions.tex <==
% 2014 written by S V N Vishwanathan (vishy@stat.purdue.edu)
% 2017 modified by Jiasen Yang (jiaseny@purdue.edu)

\RequirePackage{latexsym}
\RequirePackage{amsmath}
% \RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}
\RequirePackage[mathscr]{euscript}

\newcommand{\D}{\text{d}}
\newcommand{\ex}{\mathbb{E}}
\newcommand{\Ex}[1]{\mbox{}\mathbb{E}\left[#1\right]}
\newcommand{\Var}[1]{\mbox{}\mathrm{Var}\left(#1\right)}
\newcommand{\Cov}[1]{\mbox{}\textup{Cov}\left(#1\right)}
\newcommand{\Tr}[1]{\mbox{}\mathrm{tr}\left(#1\right)}
\newcommand{\Trsq}[1]{\mbox{}\mathrm{tr}^2\left(#1\right)}
% \newcommand{\pr}{\mathbb{P}}
\newcommand{\pr}[1]{\mbox{}\mathbb{P}\left(#1\right)}
\newcommand{\kl}[2]{\mbox{}\mathbb{KL}\left(#1\,||\,#2\right)}
\newcommand{\tAb}{\widetilde{\Ab}}
\newcommand{\tp}{\widetilde{p}}
\newcommand{\ts}{\mathsf{T}}
% \newcommand{\ts}{\top}
% \newcommand{\ind}[1]{\mathbb{I}\{#1\}}
\newcommand{\ind}[1]{\mathds{1}\{#1\}}
\newcommand{\nnz}[1]{\mathrm{nnz}(#1)}
\newcommand{\Diag}[1]{\diag \left\{#1\right\}} % pseudoinverse
\newcommand{\Pinv}[1]{\mbox{}\left(#1\right)^{\dagger}} % pseudoinverse
\newcommand{\inv}[1]{\mbox{}\left(#1\right)^{-1}} % pseudoinverse
\newcommand{\RR}[2]{\mathbb{R}^{#1 \times #2}} % Real numbers
\newcommand{\R}[1]{\mathbb{R}^{#1}} % Real numbers
\newcommand{\Sqrt}[1]{#1^{\nicefrac{1}{2}}} % pseudoinverse
\newcommand{\defeq}{\triangleq}
% \newcommand{\var}{\text{var}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\disteq}{\stackrel{d}{=}}
\newcommand{\deriv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\todo}[1]{\textcolor{red}{\texttt{TODO}: \emph{#1}}}


%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\abtil}{\tilde{\ab}}
\newcommand{\bbtil}{\tilde{\bb}}
\newcommand{\cbtil}{\tilde{\cbb}}
\newcommand{\dbtil}{\tilde{\db}}
\newcommand{\ebtil}{\tilde{\eb}}
\newcommand{\fbtil}{\tilde{\fb}}
\newcommand{\gbtil}{\tilde{\gb}}
\newcommand{\hbtil}{\tilde{\hb}}
\newcommand{\ibtil}{\tilde{\ib}}
\newcommand{\jbtil}{\tilde{\jb}}
\newcommand{\kbtil}{\tilde{\kb}}
\newcommand{\lbtil}{\tilde{\lb}}
\newcommand{\mbtil}{\tilde{\mb}}
\newcommand{\nbtil}{\tilde{\nbb}}
\newcommand{\obtil}{\tilde{\ob}}
\newcommand{\pbtil}{\tilde{\pb}}
\newcommand{\qbtil}{\tilde{\qb}}
\newcommand{\rbtil}{\tilde{\rb}}
\newcommand{\sbtil}{\tilde{\sbb}}
\newcommand{\tbtil}{\tilde{\tb}}
\newcommand{\ubtil}{\tilde{\ub}}
\newcommand{\vbtil}{\tilde{\vb}}
\newcommand{\wbtil}{\tilde{\wb}}
\newcommand{\xbtil}{\tilde{\xb}}
\newcommand{\ybtil}{\tilde{\yb}}
\newcommand{\zbtil}{\tilde{\zb}}

\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}

\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}

\newcommand{\abhat}{\hat{\ab}}
\newcommand{\bbhat}{\hat{\bb}}
\newcommand{\cbhat}{\hat{\cbb}}
\newcommand{\dbhat}{\hat{\db}}
\newcommand{\ebhat}{\hat{\eb}}
\newcommand{\fbhat}{\hat{\fb}}
\newcommand{\gbhat}{\hat{\gb}}
\newcommand{\hbhat}{\hat{\hb}}
\newcommand{\ibhat}{\hat{\ib}}
\newcommand{\jbhat}{\hat{\jb}}
\newcommand{\kbhat}{\hat{\kb}}
\newcommand{\lbhat}{\hat{\lb}}
\newcommand{\mbhat}{\hat{\mb}}
\newcommand{\nbhat}{\hat{\nb}}
\newcommand{\obhat}{\hat{\ob}}
\newcommand{\pbhat}{\hat{\pb}}
\newcommand{\qbhat}{\hat{\qb}}
\newcommand{\rbhat}{\hat{\rb}}
\newcommand{\sbhat}{\hat{\sb}}
\newcommand{\tbhat}{\hat{\tb}}
\newcommand{\ubhat}{\hat{\ub}}
\newcommand{\vbhat}{\hat{\vb}}
\newcommand{\wbhat}{\hat{\wb}}
\newcommand{\xbhat}{\widehat{\xb}}
\newcommand{\ybhat}{\hat{\yb}}
\newcommand{\zbhat}{\hat{\zb}}

\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}

\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\hbr}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\obar}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}

\newcommand{\abbar}{\bar{\ab}}
\newcommand{\bbbar}{\bar{\bb}}
\newcommand{\cbbar}{\bar{\cb}}
\newcommand{\dbbar}{\bar{\db}}
\newcommand{\ebbar}{\bar{\eb}}
\newcommand{\fbbar}{\bar{\fb}}
\newcommand{\gbbar}{\bar{\gb}}
\newcommand{\hbbar}{\bar{\hb}}
\newcommand{\ibbar}{\bar{\ib}}
\newcommand{\jbbar}{\bar{\jb}}
\newcommand{\kbbar}{\bar{\kb}}
\newcommand{\lbbar}{\bar{\lb}}
\newcommand{\mbbar}{\bar{\mb}}
\newcommand{\nbbar}{\bar{\nbb}}
\newcommand{\obbar}{\bar{\ob}}
\newcommand{\pbbar}{\bar{\pb}}
\newcommand{\qbbar}{\bar{\qb}}
\newcommand{\rbbar}{\bar{\rb}}
\newcommand{\sbbar}{\bar{\sbb}}
\newcommand{\tbbar}{\bar{\tb}}
\newcommand{\ubbar}{\bar{\ub}}
\newcommand{\vbbar}{\bar{\vb}}
\newcommand{\wbbar}{\bar{\wb}}
\newcommand{\xbbar}{\bar{\xb}}
\newcommand{\ybbar}{\bar{\yb}}
\newcommand{\zbbar}{\bar{\zb}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

% \newcommand{\Abtil}{\tilde{\Ab}}
\newcommand{\Abtil}{\widetilde{\Ab}}
\newcommand{\Bbtil}{\tilde{\Bb}}
\newcommand{\Cbtil}{\tilde{\Cb}}
\newcommand{\Dbtil}{\tilde{\Db}}
\newcommand{\Ebtil}{\tilde{\Eb}}
\newcommand{\Fbtil}{\tilde{\Fb}}
\newcommand{\Gbtil}{\tilde{\Gb}}
\newcommand{\Hbtil}{\tilde{\Hb}}
\newcommand{\Ibtil}{\tilde{\Ib}}
\newcommand{\Jbtil}{\tilde{\Jb}}
\newcommand{\Kbtil}{\tilde{\Kb}}
\newcommand{\Lbtil}{\tilde{\Lb}}
\newcommand{\Mbtil}{\tilde{\Mb}}
\newcommand{\Nbtil}{\tilde{\Nb}}
\newcommand{\Obtil}{\tilde{\Ob}}
\newcommand{\Pbtil}{\tilde{\Pb}}
\newcommand{\Qbtil}{\tilde{\Qb}}
\newcommand{\Rbtil}{\tilde{\Rb}}
\newcommand{\Sbtil}{\tilde{\Sb}}
\newcommand{\Tbtil}{\tilde{\Tb}}
\newcommand{\Ubtil}{\tilde{\Ub}}
\newcommand{\Vbtil}{\tilde{\Vb}}
\newcommand{\Wbtil}{\tilde{\Wb}}
\newcommand{\Xbtil}{\tilde{\Xb}}
\newcommand{\Ybtil}{\tilde{\Yb}}
\newcommand{\Zbtil}{\tilde{\Zb}}

\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\Zbar}{\bar{Z}}

\newcommand{\Abbar}{\bar{\Ab}}
\newcommand{\Bbbar}{\bar{\Bb}}
\newcommand{\Cbbar}{\bar{\Cb}}
\newcommand{\Dbbar}{\bar{\Db}}
\newcommand{\Ebbar}{\bar{\Eb}}
\newcommand{\Fbbar}{\bar{\Fb}}
\newcommand{\Gbbar}{\bar{\Gb}}
\newcommand{\Hbbar}{\bar{\Hb}}
\newcommand{\Ibbar}{\bar{\Ib}}
\newcommand{\Jbbar}{\bar{\Jb}}
\newcommand{\Kbbar}{\bar{\Kb}}
\newcommand{\Lbbar}{\bar{\Lb}}
\newcommand{\Mbbar}{\bar{\Mb}}
\newcommand{\Nbbar}{\bar{\Nb}}
\newcommand{\Obbar}{\bar{\Ob}}
\newcommand{\Pbbar}{\bar{\Pb}}
\newcommand{\Qbbar}{\bar{\Qb}}
\newcommand{\Rbbar}{\bar{\Rb}}
\newcommand{\Sbbar}{\bar{\Sb}}
\newcommand{\Tbbar}{\bar{\Tb}}
\newcommand{\Ubbar}{\bar{\Ub}}
\newcommand{\Vbbar}{\bar{\Vb}}
\newcommand{\Wbbar}{\bar{\Wb}}
\newcommand{\Xbbar}{\bar{\Xb}}
\newcommand{\Ybbar}{\bar{\Yb}}
\newcommand{\Zbbar}{\bar{\Zb}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\Abhat}{\hat{\Ab}}
\newcommand{\Bbhat}{\hat{\Bb}}
\newcommand{\Cbhat}{\hat{\Cb}}
\newcommand{\Dbhat}{\hat{\Db}}
\newcommand{\Ebhat}{\hat{\Eb}}
\newcommand{\Fbhat}{\hat{\Fb}}
\newcommand{\Gbhat}{\hat{\Gb}}
\newcommand{\Hbhat}{\hat{\Hb}}
\newcommand{\Ibhat}{\hat{\Ib}}
\newcommand{\Jbhat}{\hat{\Jb}}
\newcommand{\Kbhat}{\hat{\Kb}}
\newcommand{\Lbhat}{\hat{\Lb}}
\newcommand{\Mbhat}{\hat{\Mb}}
\newcommand{\Nbhat}{\hat{\Nb}}
\newcommand{\Obhat}{\hat{\Ob}}
\newcommand{\Pbhat}{\hat{\Pb}}
\newcommand{\Qbhat}{\hat{\Qb}}
\newcommand{\Rbhat}{\hat{\Rb}}
\newcommand{\Sbhat}{\hat{\Sb}}
\newcommand{\Tbhat}{\hat{\Tb}}
\newcommand{\Ubhat}{\hat{\Ub}}
\newcommand{\Vbhat}{\hat{\Vb}}
\newcommand{\Wbhat}{\hat{\Wb}}
\newcommand{\Xbhat}{\hat{\Xb}}
\newcommand{\Ybhat}{\hat{\Yb}}
\newcommand{\Zbhat}{\hat{\Zb}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\Ascr}{\mathscr{A}}
\newcommand{\Bscr}{\mathscr{B}}
\newcommand{\Cscr}{\mathscr{C}}
\newcommand{\Dscr}{\mathscr{D}}
\newcommand{\Escr}{\mathscr{E}}
\newcommand{\Fscr}{\mathscr{F}}
\newcommand{\Gscr}{\mathscr{G}}
\newcommand{\Hscr}{\mathscr{H}}
\newcommand{\Iscr}{\mathscr{I}}
\newcommand{\Jscr}{\mathscr{J}}
\newcommand{\Kscr}{\mathscr{K}}
\newcommand{\Lscr}{\mathscr{L}}
\newcommand{\Mscr}{\mathscr{M}}
\newcommand{\Nscr}{\mathscr{N}}
\newcommand{\Oscr}{\mathscr{O}}
\newcommand{\Pscr}{\mathscr{P}}
\newcommand{\Qscr}{\mathscr{Q}}
\newcommand{\Rscr}{\mathscr{R}}
\newcommand{\Sscr}{\mathscr{S}}
\newcommand{\Tscr}{\mathscr{T}}
\newcommand{\Uscr}{\mathscr{U}}
\newcommand{\Vscr}{\mathscr{V}}
\newcommand{\Wscr}{\mathscr{W}}
\newcommand{\Xscr}{\mathscr{X}}
\newcommand{\Yscr}{\mathscr{Y}}
\newcommand{\Zscr}{\mathscr{Z}}

\newcommand{\Ascrb}{\boldsymbol{\Ascr}}
\newcommand{\Bscrb}{\boldsymbol{\Bscr}}
\newcommand{\Cscrb}{\boldsymbol{\Cscr}}
\newcommand{\Dscrb}{\boldsymbol{\Dscr}}
\newcommand{\Escrb}{\boldsymbol{\Escr}}
\newcommand{\Fscrb}{\boldsymbol{\Fscr}}
\newcommand{\Gscrb}{\boldsymbol{\Gscr}}
\newcommand{\Hscrb}{\boldsymbol{\Hscr}}
\newcommand{\Iscrb}{\boldsymbol{\Iscr}}
\newcommand{\Jscrb}{\boldsymbol{\Jscr}}
\newcommand{\Kscrb}{\boldsymbol{\Kscr}}
\newcommand{\Lscrb}{\boldsymbol{\Lscr}}
\newcommand{\Mscrb}{\boldsymbol{\Mscr}}
\newcommand{\Nscrb}{\boldsymbol{\Nscr}}
\newcommand{\Oscrb}{\boldsymbol{\Oscr}}
\newcommand{\Pscrb}{\boldsymbol{\Pscr}}
\newcommand{\Qscrb}{\boldsymbol{\Qscr}}
\newcommand{\Rscrb}{\boldsymbol{\Rscr}}
\newcommand{\Sscrb}{\boldsymbol{\Sscr}}
\newcommand{\Tscrb}{\boldsymbol{\Tscr}}
\newcommand{\Uscrb}{\boldsymbol{\Uscr}}
\newcommand{\Vscrb}{\boldsymbol{\Vscr}}
\newcommand{\Wscrb}{\boldsymbol{\Wscr}}
\newcommand{\Xscrb}{\boldsymbol{\Xscr}}
\newcommand{\Xscrbh}{\hat{\Xscrb}}
\newcommand{\Yscrb}{\boldsymbol{\Yscr}}
\newcommand{\Zscrb}{\boldsymbol{\Zscr}}

\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}
\newcommand{\Mtilde}{\widetilde{M}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}

\newcommand{\avec}{\vec{a}}
\newcommand{\bvec}{\vec{b}}
\newcommand{\cvec}{\vec{c}}
\newcommand{\dvec}{\vec{d}}
\newcommand{\evec}{\vec{e}}
\newcommand{\fvec}{\vec{f}}
\newcommand{\gvec}{\vec{g}}
\newcommand{\hvec}{\vec{h}}
\newcommand{\ivec}{\vec{i}}
\newcommand{\jvec}{\vec{j}}
\newcommand{\kvec}{\vec{k}}
\newcommand{\lvec}{\vec{l}}
\newcommand{\mvec}{\vec{m}}
\newcommand{\nvec}{\vec{n}}
\newcommand{\ovec}{\vec{o}}
\newcommand{\pvec}{\vec{p}}
\newcommand{\qvec}{\vec{q}}
\newcommand{\rvec}{\vec{r}}
\newcommand{\svec}{\vec{s}}
\newcommand{\tvec}{\vec{t}}
\newcommand{\uvec}{\vec{u}}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}

\newcommand{\va}{\vec{a}}
\newcommand{\vecb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vd}{\vec{d}}
\newcommand{\veee}{\vec{e}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vg}{\vec{g}}
\newcommand{\vh}{\vec{h}}
\newcommand{\vi}{\vec{i}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vp}{\vec{p}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vr}{\vec{r}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vz}{\vec{z}}

\newcommand{\Avec}{\vec{A}}
\newcommand{\Bvec}{\vec{B}}
\newcommand{\Cvec}{\vec{C}}
\newcommand{\Dvec}{\vec{D}}
\newcommand{\Evec}{\vec{E}}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\Gvec}{\vec{G}}
\newcommand{\Hvec}{\vec{H}}
\newcommand{\Ivec}{\vec{I}}
\newcommand{\Jvec}{\vec{J}}
\newcommand{\Kvec}{\vec{K}}
\newcommand{\Lvec}{\vec{L}}
\newcommand{\Mvec}{\vec{M}}
\newcommand{\Nvec}{\vec{N}}
\newcommand{\Ovec}{\vec{O}}
\newcommand{\Pvec}{\vec{P}}
\newcommand{\Qvec}{\vec{Q}}
\newcommand{\Rvec}{\vec{R}}
\newcommand{\Svec}{\vec{S}}
\newcommand{\Tvec}{\vec{T}}
\newcommand{\Uvec}{\vec{U}}
\newcommand{\Vvec}{\vec{V}}
\newcommand{\Wvec}{\vec{W}}
\newcommand{\Xvec}{\vec{X}}
\newcommand{\Yvec}{\vec{Y}}
\newcommand{\Zvec}{\vec{Z}}

\newcommand{\Amat}{\Ab}
\newcommand{\Bmat}{\Bb}
\newcommand{\Cmat}{\Cb}
\newcommand{\Dmat}{\Db}
\newcommand{\Emat}{\Eb}
\newcommand{\Fmat}{\Fb}
\newcommand{\Gmat}{\Gb}
\newcommand{\Hmat}{\Hb}
\newcommand{\Imat}{\Ib}
\newcommand{\Lmat}{\Lb}

\newcommand{\Vmat}{\Vb}
\newcommand{\Wmat}{\Wb}
\newcommand{\Xmat}{\Xb}
\newcommand{\Ymat}{\Yb}
\newcommand{\Zmat}{\Zb}


\newcommand{\yvecbar}{\bar{\vec{y}}}
\newcommand{\wvecbar}{\bar{\vec{w}}}
\newcommand{\xvecbar}{\bar{\vec{x}}}
\newcommand{\yvectil}{\tilde{\vec{y}}}
\newcommand{\yvechat}{\hat{\vec{y}}}

\newcommand{\vol}{\text{vol}}


%%%%%%%% Theorems and Friends %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
\fi

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi

\ifx\example\undefined
\newtheorem{example}{Example}
\fi

\ifx\property\undefined
\newtheorem{property}{Property}
\fi

\ifx\lemma\undefined
\newtheorem{lemma}[theorem]{Lemma}
\fi

\ifx\proposition\undefined
\newtheorem{proposition}[theorem]{Proposition}
\fi

\ifx\remark\undefined
\newtheorem{remark}[theorem]{Remark}
\fi

\ifx\corollary\undefined
\newtheorem{corollary}[theorem]{Corollary}
\fi

\ifx\definition\undefined
\newtheorem{definition}{Definition}
\fi

\ifx\conjecture\undefined
\newtheorem{conjecture}[theorem]{Conjecture}
\fi

\ifx\axiom\undefined
\newtheorem{axiom}[theorem]{Axiom}
\fi

\ifx\claim\undefined
\newtheorem{claim}[theorem]{Claim}
\fi

\ifx\assumption\undefined
\newtheorem{assumption}[theorem]{Assumption}
\fi

% \renewcommand{\qedsymbol}{$\blacksquare$}


%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\FF}{\mathbb{F}} % Fexpectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
% \newcommand{\RR}{\mathbb{R}} % Real numbers
\newcommand{\RRbar}{\overline{\RR}} % Real numbers
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}} % Integers

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\intdim}{\mathop{\mathrm{intdim}}}
\newcommand{\sr}{\mathop{\mathrm{sr}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\ri}{\mathop{\mathrm{ri}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\bd}{\mathop{\mathrm{bd}}}
\newcommand{\emp}{\mathop{\mathrm{emp}}}
\newcommand{\core}{\mathop{\mathrm{core}}}
\newcommand{\co}{\mathop{\mathrm{co}}}
% \newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\eproof}{$\null\hfill\blacksquare$}

%\newcommand{\ln}{\mathop{\mathrm{ln}}}
%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}
%%%%%%%% Short Forms %%%%%%%%%%%%%%%

\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\emph{i.i.d.}}
\newcommand{\wrt}{\emph{w.r.t.}\ }
\newcommand{\cf}{\emph{cf.}\ }

%%%%%%%% Brackets %%%%%%%%%%%%%%%

\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\|#1\|}
% \newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}

%%%%%%%%%%%%%%%  Mathematical Constants  %%%%%%%%%%%%%%%

\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
% \newcommand{\ind}{\boldsymbol{\mathsf{I}}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\sqrttwo}{\sqrt{2}}
\newcommand{\invsqrttwo}{\frac{1}{\sqrt{2}}}
\newcommand{\rmd}{\ensuremath{\mathrm{d}}}

%%%%%%%% Greek Symbols %%%%%%%%%%%%%%%

\newcommand{\sigmab}{\bm{\sigma}}
\newcommand{\Lambdab}{\mathbf{\Lambda}}
\newcommand{\Sigmab}{\mathbf{\Sigma}}
\newcommand{\Thetab}{\mathbf{\Theta}}

\newcommand{\val}{\vec{\alpha}}
\newcommand{\vbeta}{\vec{\beta}}
\newcommand{\vde}{\vec{\delta}}
\newcommand{\vga}{\vec{\gamma}}
\newcommand{\vsig}{\vec{\sigma}}
\newcommand{\vth}{\vec{\theta}}
\newcommand{\veta}{\vec{\eta}}
\newcommand{\vnu}{\vec{\nu}}
\newcommand{\vpsi}{\vec{\psi}}
\newcommand{\vpi}{\vec{\pi}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\vxi}{\vec{\xi}}
\newcommand{\vze}{\vec{\zeta}}

\newcommand{\valbar}{\bar{\val}}
\newcommand{\valhat}{\hat{\val}}
\newcommand{\valtil}{\tilde{\val}}
\newcommand{\vthtil}{\tilde{\vth}}
\newcommand{\vthhat}{\hat{\vth}}
\newcommand{\vthbar}{\bar{\vth}}
\newcommand{\vbetatil}{\tilde{\vbeta}}
\newcommand{\vbetahat}{\hat{\vbeta}}

\newcommand{\alphavec}{\val}
\newcommand{\alphavecbar}{\bar{\val}}
\newcommand{\alphavechat}{\hat{\val}}
\newcommand{\alphavectil}{\tilde{\val}}
\newcommand{\betavec}{\vec{\beta}}
\newcommand{\gammavec}{\vec{\gamma}}
\newcommand{\deltavec}{\vec{\delta}}
\newcommand{\etavec}{\vec{\eta}}
\newcommand{\phivec}{\vec{\phi}}
\newcommand{\psivec}{\vec{\psi}}
\newcommand{\thetavec}{\vec{\theta}}
\newcommand{\muvec}{\vec{\mu}}
\newcommand{\xivec}{\vec{\xi}}
\newcommand{\chivec}{\vec{\chi}}
\newcommand{\lambdavec}{\vec{\lambda}}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\pitil}{\tilde{\pi}}
\newcommand{\elltil}{\tilde{\ell}}
\newcommand{\rhob}{\boldsymbol{\rho}}
\newcommand{\Omegab}{\boldsymbol{\Omega}}
\newcommand{\Phib}{\boldsymbol{\Phi}}

\newcommand{\delhat}{\hat{\delta}}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\delbar}{\bar{\delta}}
\newcommand{\alphahat}{\hat{\alpha}}
\newcommand{\alphatil}{\tilde{\alpha}}
\newcommand{\mubar}{\bar{\mu}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\bar{\theta}}
\newcommand{\betahat}{\hat{\beta}}

\newcommand{\xibar}{\bar{\xi}}
\newcommand{\lambdavectil}{\tilde{\vec{\lambda}}}
\newcommand{\thetatil}{\tilde{\theta}}
\newcommand{\betatil}{\tilde{\beta}}

%%%%%%%% Various Optimizers %%%%%%%%%%%%%%%

\newcommand{\BMRM}{{\sf BMRM}}
\newcommand{\bmrm}{{\sf BMRM}}
\newcommand{\cpm}{{\sf CPM}}
\newcommand{\liblinear}{{\sf liblinear}}
\newcommand{\lsbmrm}{{\sf ls-bmrm}}
\newcommand{\qpbmrm}{{\sf qp-bmrm}}
\newcommand{\pegasos}{{\sf pegasos}}
\newcommand{\pegan}{{\sf pegasos-$n$}}
\newcommand{\pegaone}{{\sf pegasos-1}}
\newcommand{\svmstruct}{{\sf SVM-Struct}}
\newcommand{\svmperf}{{\sf SVM-Perf}}
\newcommand{\nest}{{\sf pragam}}
\newcommand{\nestb}{{\sf pragam-b}}
\newcommand{\mcn}{{\sf M$^3$N}}
\newcommand{\expgrad}{{\sf ExpGrad}}
\newcommand{\smo}{{\sf SMO}}
\newcommand{\lasvm}{{\sf LaSVM}}
\newcommand{\sms}{{\sf SMS}}


\newcommand{\prbep}{{\sf PRBEP}}
\newcommand{\rocarea}{{\sf ROCArea}}

\newcommand{\arow}[2]{#1_{#2\cdot}}
\newcommand{\acol}[2]{#1_{\cdot#2}}
\newcommand{\expunder}[1]{\mathop{\EE}\limits_{#1}}
\newcommand{\mean}[1]{\mathop{\EE}\sbr{{#1}}}
\newcommand{\vars}[2]{\var_{{#1}}\sbr{{#2}}}
\newcommand{\expec}[2]{\mathop{\EE}_{{#1}}\sbr{{#2}}}

\newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}
\def\ci{\perp\!\!\!\perp}

\newcommand{\ve}{\varepsilon}

\newcommand{\gstar}{g^{\star}}
\newcommand{\fstar}{f^{\star}}
\newcommand{\hstar}{h^{\star}}
\newcommand{\Astar}{A^{\star}}
\newcommand{\Kstar}{K^{\star}}

\newcommand{\var}{\mathrm{Var}}
\newcommand{\grad}{{\nabla}}
\newcommand{\gradtil}{{\tilde{\grad}}}
\newcommand{\MED}{{\text{MED}}}
\newcommand{\where}{{\quad \text{where} \quad}}
\newcommand{\lcg}{{\textit{l.c.g}}}
\newcommand{\cp}{\mathrm{cp}}
\newcommand{\err}{{\sf err}}
\newcommand{\wvechat}{\hat{\vec{w}}}

\newcommand{\ydiff}[2]{\delta(#1, #2)}
\newcommand{\ykdiff}[2]{\delta(#1, #2)^{\kappa}}
\newcommand{\myfdiff}[2]{\Delta f(#1, #2)}


\newcommand{\Aone}{\textbf{A1}}
\newcommand{\Atwo}{\textbf{A2}}

%%%%%%%% Modifications to Algorithmic %%%%%%%%%%%%%%%
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}




==> Proof_of_lowrank_lev_score.tex <==
%!TEX root = nips_LDA.tex

\section{Proof of Theorem~\ref{thm:psiterative}}

Using the quantities defined in Algorithm~\ref{algo:psiterative}, let
%
\begin{flalign}\label{eqn:pspdits}
\Fb^{(j)}=\Ab_{k}^\ts(\Ab_{k}\Ab_{k}^\ts)^{\dagger}\Lb^{(j)}.
\end{flalign}
%
for $j=1,\dots, t$.

Note that $\Fb=\Fb^{(1)}$. Our next result provides an alternative expression for $\Fb^{(j)}$ which is easier to work with. We remind the reader that $\Ub_{k} \in \mathbb{R}^{n \times k}$, $\Vb_{k} \in \mathbb{R}^{d \times k}$ and $\Sigmab_{k} \in \mathbb{R}^{k \times k}$ are, respectively, the matrices of the left singular vectors, right singular vectors  and singular values of $\Ab_{k}$.


\begin{lemma}\label{lem:psalt_xopt}
	For $j=1,2,\dots ,t$, let $\Lb^{(j)}$ be the intermediate matrices in Algorithm~\ref{algo:psiterative} and $\Fb^{(j)}$ be the matrix defined in eqn.~\eqref{eqn:pspdits}.
	Then for any $j=1,2,\dots ,t$, $\Fb^{(j)}$ can also be expressed as
	\begin{flalign}
	\Fb^{(j)}=\Vb_{k}\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}\nonumber
	\end{flalign}
\end{lemma}

\begin{proof}
	Using the thin SVD representation of $\Ab_{k}$ we have
	\begin{flalign}
	\Fb^{(j)}=&~\Vb_{k}\Sigmab_{k}\Ub_{k}^\ts(\Ub_{k}\Sigmab_{k}^2\Ub_{k}^\ts)^{\dagger}\Lb^{(j)}
	=~\Vb_{k}\Sigmab_{k}\Ub_{k}^\ts\Ub_{k}\Sigmab_{k}^{-2}\Ub_{k}^\ts\Lb^{(j)}\nonumber\\
	=&~\Vb_{k}\Sigmab_{k}\Sigmab_{k}^{-2}\Ub_{k}^\ts\Lb^{(j)}=~\Vb_{k}\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}\label{eq:psfda11}
	\end{flalign}	
\end{proof}

Our next result provides a bound which later on plays a very important role in showing that the underlying error decays exponentially as the number of iterations in Algorithm~\ref{algo:psiterative} increases.

\begin{lemma}\label{lem:psstruct2}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	For $j=1,2,\dots ,t$, let $\Lb^{(j)}$ and $\widetilde{\Fb}^{(j)}$ be the intermediate matrices in Algorithm~\ref{algo:psiterative}, $\Fb^{(j)}$ be the matrix defined in eqn.~\eqref{eqn:pspdits} and $\Sb_j\in\RR{d}{s}$ be the sketching matrix. If eqn.~\eqref{eq:psstruct1} is satisfied then for all $j=1,\dots, t$
	\begin{flalign}
	\nbr{(\wb-\mb)^\ts(\widetilde{\Fb}^{(j)}-\Fb^{(j)})}_2\le~\ve\nbr{\alphab_{k}}_2\nbr{\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}}_2 \,.
	\end{flalign}
	%
\end{lemma}

\begin{proof}
	Using \textit{Weyl's inequality} and combining eqn.~\eqref{eq:psstruct1} and the fact $\ve<1$, we have, for all $i=1,2,\dots,k$,
	\begin{flalign}
	&\abs{\sigma_i^2(\Vb_{k}^\ts\Sb_{j})-1}\le\nbr{\Vb_{k}^\ts\Sb_{j}\Sb_{j}^\ts\Vb_{k}-\Ib_k}_2\le~\frac{\ve}{2}\le\frac{1}{2}\nonumber\\
	\implies&~\frac{1}{2}\le\sigma_i^2(\Vb_{k}^\ts\Sb_{j})\le\frac{3}{2}\label{eq:psweyl}
	\end{flalign}
	Thus, all the singular values of $\Vb_{k}^\ts\Sb_{j}$ are strictly positive and hence it has full-rank equal to $k$. Again, using eqn.~\eqref{eq:psweyl}
	\begin{flalign}
	\abs{1-\sigma_i^{-2}(\Vb_{k}^\ts\Sb_{j})}\le\frac{\abs{\sigma_i^{2}(\Vb_{k}^\ts\Sb_{j})-1}}{\sigma_i^{2}(\Vb_{k}^\ts\Sb_{j})}\le\frac{\ve/2}{1/2}=\ve\label{eq:psweyl2}
	\end{flalign}
	
	Using SVD of $\Ab_{k}$, we express $\widetilde{\Fb}^{(j)}$ in terms of $\Fb^{(j)}$.
	\begin{flalign}
	\widetilde{\Fb}^{(j)}=&~\Vb_{k}\Sigmab_{k}\Ub_{k}^\ts(\Ub_{k}\Sigmab_{k}\Vb_{k}^\ts\Sb_{j})^{\dagger\ts}(\Ub_{k}\Sigmab_{k}\Vb_{k}^\ts\Sb_{j})^{\dagger}\Lb^{(j)}\nonumber\\
	=&~\Vb_{k}\Sigmab_{k}\Ub_{k}^\ts\left((\Vb_{k}^\ts\Sb_{j})^\dagger\Sigmab_{k}^{-1}\Ub_{k}^\ts\right)^{\ts}\left((\Vb_{k}^\ts\Sb_{j})^\dagger\Sigmab_{k}^{-1}\Ub_{k}^\ts\right)\Lb^{(j)}\nonumber\\
	=&~\Vb_{k}\Sigmab_{k}\Ub_{k}^\ts\Ub_{k}\Sigmab_{k}^{-1}(\Vb_{k}^\ts\Sb_{j})^{\dagger\ts}(\Vb_{k}^\ts\Sb_{j})^\dagger\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}\nonumber\\
	=&~\Vb_{k}(\Vb_{k}^\ts\Sb_{j})^{\dagger\ts}(\Vb_{k}^\ts\Sb_{j})^\dagger\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}\label{eq:psfda1}
	\end{flalign}
	In the above derivations, we have used the fact that $\Vb_{k}^\ts\Sb_j$ has the full rank in order to simplify the pseudo-inverse. Now, let $\widetilde{\Eb}_{j}=(\Vb_{k}^\ts\Sb_j)^{\dagger\ts}(\Vb_{k}^\ts\Sb_j)^{\dagger}-\Ib_{k}$ and we rewrite eqn.~\eqref{eq:psfda1} as
	\begin{flalign}
	\widetilde{\Fb}^{(j)}=&~\Vb_{k}(\Ib_{k}+\widetilde{\Eb}_j)\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}=~\Vb_{k}\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}+~\Vb_{k}\widetilde{\Eb}_j\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}\nonumber\\
	=&~\Fb^{(j)}+~\Vb_{k}\widetilde{\Eb}_j\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}\label{eq:psfda05}
	\end{flalign}
	where eqn.~\eqref{eq:psfda05} follows from Lemma~\ref{lem:psalt_xopt}.
	
	Now, note that, eqn.~\eqref{eq:psweyl2} and the fact $\Vb_{k}^\ts\Sb_{j}$ has full rank imply
	\begin{flalign}
	\nbr{\widetilde{\Eb}_j}_2=\nbr{\Ib_{k}-(\Vb_{k}^\ts\Sb_j)^{\dagger\ts}(\Vb_{k}^\ts\Sb_j)^{\dagger}}_2=\max_{1\le i\le k}	\abs{1-\sigma_i^{-2}(\Vb_{k}^\ts\Sb_{j})}\le\ve\label{eq:psfda06}
	\end{flalign}
	
	
	Next, we combine eqns.~\eqref{eq:psfda05} and \eqref{eq:psfda06} to have
	\begin{flalign}
	\nbr{(\wb-\mb)^\ts(\widetilde{\Fb}^{(j)}-\Fb^{(j)})}_2=&~\nbr{(\wb-\mb)^\ts\Vb_{k}\widetilde{\Eb}_j\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}}_2\nonumber\\
	\le&~\nbr{(\wb-\mb)^\ts\Vb_{k}}_2\nbr{\widetilde{\Eb}_j}_2\nbr{\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}}_2\nonumber\\
	\le&~\ve~\nbr{(\wb-\mb)^\ts\Vb_{k}}_2\nbr{\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}}_2\nonumber\\
	=&~\ve~\nbr{(\wb-\mb)^\ts\Vb_{k}\Vb_{k}^\ts}_2\nbr{\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}}_2\nonumber\\
	=&~\ve~\nbr{\alphab_{k}}_2\nbr{\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}}_2\label{eq:psfda015}
	%\le&~\ve~\nbr{\alphab_{k}}_2~\frac{1}{2\sqrt{\lambda}}=\frac{\ve}{\sqrt{\lambda}}\nbr{\alphab_{k}}_2\label{eq:rfda9}
	%=&~2\ve~\nbr{(\wb-\mb)^\ts\Vb_{k}}_2=~2\ve~\nbr{\alphab_{k}}_2
	\end{flalign}
	where the first inequality follows from the submultiplicativity  and the second last equality holds due to unitary invariance of spectral-norm. 
	This concludes the proof.
\end{proof}

The next lemma presents a structural result for the matrix $\Fb$.
%
\begin{lemma}\label{lem:psinduction}
	Let $\widetilde{\Fb}^{(j)}$, $j=1,\dots, t$ be the sequence of matrices introduced in Algorithm~\ref{algo:psiterative} and let $\Fb^{(t)}\in\R{d}$ be defined as in eqn.~\eqref{eqn:pspdits}. Then,
	\begin{flalign}
	\Fb=\Fb^{(t)}+\sum_{j=1}^{t-1}\widetilde{\Fb}^{(j)},\label{eq:psiterative2_1}
	\end{flalign}
	where $\Fb$ is given by eqn.~\eqref{eq:psrfda3}.
\end{lemma}

\begin{proof}
	We prove by induction on $t$.
	
	\medspace
	
	Note that, $\Lb^{(1)}=\Omegab$. So, for $t=1$, eqn.~\eqref{eqn:pspdits} boils down to $$\Fb^{(1)}=\Ab_{k}^\ts(\Ab_{k}\Ab_{k}^\ts)^{\dagger}\Lb^{(1)}=\Fb. $$
	
	For $t=2$, we have
	\begin{flalign}
	\Fb^{(2)}
	=&~\Ab_{k}^\ts(\Ab_{k}\Ab_{k}^\ts)^{\dagger}\Lb^{(2)}\nonumber\\
	=&~\Ab_{k}^\ts(\Ab_{k}\Ab_{k}^\ts)^{\dagger}\left(\Lb^{(1)}-\Ab_{k}\widetilde{\Fb}^{(1)}\right)\nonumber\\
	=&~\Ab_{k}^\ts(\Ab_{k}\Ab_{k}^\ts)^{\dagger}\left(\Lb^{(1)}-\Ab_{k}\Ab_{k}^\ts(\Ab_{k} \Sb_1)^{\dagger\ts}(\Ab_{k} \Sb_1)^{\dagger}\Lb^{(1)}\right)\nonumber\\
	=&~\Ab_{k}^\ts(\Ab_{k}\Ab_{k}^\ts)^{\dagger}\Lb^{(1)}-\Ab_{k}^\ts(\Ab_{k}\Ab_{k}^\ts)^{\dagger}(\Ab_{k}\Ab_{k}^\ts)(\Ab_{k} \Sb_1)^{\dagger\ts}(\Ab_{k} \Sb_1)^{\dagger}\Lb^{(1)}\label{psrfda0}
	\end{flalign}
	Using thin SVD representation of $\Ab_{k}$, we further have
	\begin{flalign}
	\Ab_{k}^\ts(\Ab_{k}\Ab_{k}^\ts)^{\dagger}(\Ab_{k}\Ab_{k}^\ts)=&~\Vb_{k}\Sigmab_{k}\Ub_{k}^\ts(\Ub_{k}\Sigmab_{k}^2\Ub_{k}^\ts)^{\dagger}\Ub_{k}\Sigmab_{k}^2\Ub_{k}^\ts
	=~\Vb_{k}\Sigmab_{k}\Ub_{k}^\ts\Ub_{k}\Sigmab_{k}^{-2}\Ub_{k}^\ts\Ub_{k}\Sigmab_{k}^2\Ub_{k}^\ts\nonumber\\
	=&~\Vb_{k}\Sigmab_{k}\Ub_{k}^\ts=~\Ab_{k}^\ts\label{psrfda01}.
	\end{flalign}
	% Thus, eqn.~\eqref{eq:iterative2_1} is satisfied for $t=1,2$.
	
	Combining eqns.~\eqref{psrfda0} and \eqref{psrfda01}, we have
	\begin{flalign*}
	\Fb^{(2)}=~\Ab_{k}^\ts(\Ab_{k}\Ab_{k}^\ts)^{\dagger}\Lb^{(1)}-\Ab_{k}^\ts(\Ab_{k} \Sb_1)^{\dagger\ts}(\Ab_{k} \Sb_1)^{\dagger}\Lb^{(1)}=~\Fb-\widetilde{\Fb}^{(1)}.
	\end{flalign*}
	
	
	Now, suppose eqn.~\eqref{eq:psiterative2_1} is also true for $t=p$, \ie,
	\begin{flalign}
	\Fb^{(p)}=\Fb-\sum_{j=1}^{p-1}\widetilde{\Fb}^{(j)}. \label{eq:psiterative2_2}
	\end{flalign}
	%
	Then, for $t=p+1$, we can express $\Fb^{(t)}$ as
	\begin{flalign}
	\Fb^{(p+1)}
	=&~\Ab_{k}^\ts(\Ab_{k}\Ab_{k}^\ts)^{\dagger}\Lb^{(p+1)}\nonumber \\
	=&~\Ab_{k}^\ts(\Ab_{k}\Ab_{k}^\ts)^{\dagger}\left(\Lb^{(p)}-\Ab_{k}\widetilde{\Fb}^{(p)}\right)\nonumber\\
	=&~\Ab_{k}^\ts(\Ab_{k}\Ab_{k}^\ts)^{\dagger}\left(\Lb^{(p)}-\Ab_{k}\Ab_{k}^\ts(\Ab_{k} \Sb_p)^{\dagger\ts}(\Ab_{k} \Sb_p)^{\dagger}\Lb^{(p)}\right)\nonumber\\
	=&~\Ab_{k}^\ts(\Ab_{k}\Ab_{k}^\ts)^{\dagger}\Lb^{(p)}-\Ab_{k}^\ts(\Ab_{k}\Ab_{k}^\ts)^{\dagger}(\Ab_{k}\Ab_{k}^\ts)(\Ab_{k} \Sb_p)^{\dagger\ts}(\Ab_{k} \Sb_p)^{\dagger}\Lb^{(p)}\nonumber\\
	=&~\Ab_{k}^\ts(\Ab_{k}\Ab_{k}^\ts)^{\dagger}\Lb^{(p)}-\Ab_{k}^\ts(\Ab_{k} \Sb_p)^{\dagger\ts}(\Ab_{k} \Sb_p)^{\dagger}\Lb^{(p)}\nonumber\\
	=&~\Fb^{(p)}-\widetilde{\Fb}^{(p)}=\left(\Fb-\sum_{j=1}^{p-1}\widetilde{\Fb}^{(j)}\right)-\widetilde{\Fb}^{(p)}=\Fb-\sum_{j=1}^{p}\widetilde{\Fb}^{(j)}
	\end{flalign}
	In the above derivation, we have used eqns.~\eqref{psrfda01} and \eqref{eq:psiterative2_2}.
	
	By the induction principle, we have proven eqn.~\eqref{eq:psiterative2_1}.
	%
\end{proof}

\begin{remark}
	Repeated application of Lemma~\ref{lem:psstruct2} and Lemma~\ref{lem:psinduction} yields:
	\begin{flalign}
	\nbr{(\wb-\mb)^\ts(\widehat{\Fb} -\Fb)}_2
	=& \nbr{(\wb-\mb)^\ts\big(\sum_{j=1}^{t}\widetilde{\Fb}^{(j)}-\Fb\big)}_2
	= \nbr{(\wb-\mb)^\ts\left(\widetilde{\Fb}^{(t)}-\big(\Fb-\sum_{j=1}^{t-1}\widetilde{\Fb}^{(j)}\big)\right)}_2\nonumber\\
	=& \nbr{(\wb-\mb)^\ts\left(\widetilde{\Fb}^{(t)}-\Fb^{(t)}\right)}_2\le~\ve~\nbr{\alphab_{k}}_2\nbr{\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(t)}}_2.\label{eq:psiter2}
	\end{flalign}
\end{remark}

The next bound provides a critical inequality that can be used recursively in order to establish Theorem~\ref{thm:psiterative}.
\begin{lemma}\label{lem:psrecur}
	Let $\Lb^{(j)}$, $j=1,\dots, t$, be the matrices of Algorithm~\ref{algo:psiterative} and $\Rb$ is as defined in Lemma~\ref{lem:psalt_xopt}. For any $j=1,\dots, t-1$, if eqn.~\eqref{eq:psstruct1} is satisfied, then
	\begin{flalign}
	&\nbr{\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j+1)}}_2\le~\ve\nbr{\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}}_2.\label{eq:psrecur}
	\end{flalign}
\end{lemma}

\begin{proof} From Algorithm~\ref{algo:psiterative}, we have for $j=1,\dots, t-1$
	\begin{flalign}
	\Lb^{(j+1)}=&~\Lb^{(j)}-\Ab_{k}\widetilde{\Fb}^{(j)}\nonumber\\
	=&~\Lb^{(j)}-\Ab_{k}\Ab_{k}^\ts(\Ab_{k} \Sb_j)^{\dagger\ts}(\Ab_{k} \Sb_j)^{\dagger}\Lb^{(j)}\label{eq:psrecur6}
	\end{flalign}
	
	Now, starting with thin SVD representation of $\Ab_{k}$, we have 
	\begin{flalign}
	&~\Ab_{k}\Ab_{k}^\ts(\Ab_{k} \Sb_j)^{\dagger\ts}(\Ab_{k} \Sb_j)^{\dagger}\Lb^{(j)}\nonumber\\
	=&~\Ub_{k}\Sigmab_{k}^2\Ub_{k}^\ts\left(\Ub_{k}\Sigmab_{k}\Vb_{k}^\ts\Sb_{j}\right)^{\dagger\ts}\left(\Ub_{k}\Sigmab_{k}\Vb_{k}^\ts\Sb_{j}\right)^{\dagger}\Lb^{(j)}\nonumber\\
	=&~\Ub_{k}\Sigmab_{k}^2\Ub_{k}^\ts\left((\Vb_{k}^\ts\Sb_{j})^\dagger\Sigmab_{k}^{-1}\Ub_{k}^\ts\right)^{\ts}\left((\Vb_{k}^\ts\Sb_{j})^\dagger\Sigmab_{k}^{-1}\Ub_{k}^\ts\right)\Lb^{(j)}\nonumber\\
	=&~\Ub_{k}\Sigmab_{k}^2\Ub_{k}^\ts\Ub_{k}\Sigmab_{k}^{-1}(\Vb_{k}^\ts\Sb_{j})^{\dagger\ts}(\Vb_{k}^\ts\Sb_{j})^\dagger\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}\nonumber\\
	=&~\Ub_{k}\Sigmab_{k}(\Vb_{k}^\ts\Sb_{j})^{\dagger\ts}(\Vb_{k}^\ts\Sb_{j})^\dagger\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}\label{eq:psrfda12}
	\end{flalign}
	In the above derivations, we have used the fact that $\Vb_{k}^\ts\Sb_j$ has the full rank (see eqn.~\eqref{eq:psweyl}) in order to simplify the pseudo-inverse. Now, let $\widetilde{\Eb}_{j}=(\Vb_{k}^\ts\Sb_j)^{\dagger\ts}(\Vb_{k}^\ts\Sb_j)^{\dagger}-\Ib_{k}$ and we rewrite eqn.~\eqref{eq:psrfda12} as
	\begin{flalign}
	~\Ab_{k}\Ab_{k}^\ts(\Ab_{k} \Sb_j)^{\dagger\ts}(\Ab_{k} \Sb_j)^{\dagger}\Lb^{(j)}
	=&~\Ub_{k}\Sigmab_{k}(\Ib_{k}+\widetilde{\Eb}_{j})\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}\nonumber\\
	=&~\Ub_{k}\Ub_{k}^\ts\Lb^{(j)}+\Ub_{k}\Sigmab_{k}\widetilde{\Eb}_{j}\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}\label{eq:psrecur10}
	\end{flalign}
	
	
	So, combining, eqns.~\eqref{eq:psrecur6} and \eqref{eq:psrecur10}
	\begin{flalign}
	\Lb^{(j+1)}=~\Lb^{(j)}-\Ub_{k}\Ub_{k}^\ts\Lb^{(j)}-\Ub_{k}\Sigmab_{k}\widetilde{\Eb}_{j}\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}\label{eq:psrecur19}
	\end{flalign}
	
	Note that, eqn.~\eqref{eq:psfda06} implies $\nbr{\widetilde{\Eb}_{j}}_2\le\ve$  using eqn.~\eqref{eq:psrecur19}
	\begin{flalign}
	\nbr{\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j+1)}}_2=&~\nbr{\Sigmab_{k}^{-1}\Ub_{k}^\ts\left(\Lb^{(j)}-\Ub_{k}\Ub_{k}^\ts\Lb^{(j)}-\Ub_{k}\Sigmab_{k}\widetilde{\Eb}_{j}\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}\right)}_2\nonumber\\
	=&~\nbr{\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}-\Sigmab_{k}^{-1}\Ub_{k}^\ts\Ub_{k}\Ub_{k}^\ts\Lb^{(j)}-\Sigmab_{k}^{-1}\Ub_{k}^\ts\Ub_{k}\Sigmab_{k}\widetilde{\Eb}_{j}\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}}_2\nonumber\\
	=&~\nbr{\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}-\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}-\widetilde{\Eb}_{j}\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}}_2\nonumber\\
	=&~\nbr{-\widetilde{\Eb}_{j}\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}}_2\le~\nbr{\widetilde{\Eb}_{j}}_2\nbr{\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}}_2\nonumber\\
	\le&~\ve\nbr{\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(j)}}_2
	\end{flalign}
	where the first inequality follows from submultiplicativity. This concludes the proof.
\end{proof}
%
\paragraph{Proof of Theorem~\ref{thm:psiterative}} Applying Lemma~\ref{lem:psrecur} iteratively, we have
\begin{flalign}
\nbr{\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(t)}}_2\le&~\ve\nbr{\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(t-1)}}_2\nonumber\\
&\vdots\nonumber\\
\le&~\ve^{t-1}\nbr{\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(1)}}_2\label{eq:psrecur71}
\end{flalign}

Now, from eqn~\eqref{eq:psrecur71}
\begin{flalign}
\nbr{\Sigmab_{k}^{-1}\Ub_{k}^\ts\Lb^{(1)}}_2=&~\nbr{\Sigmab_{k}^{-1}\Ub_{k}^\ts\Omegab}_2\nonumber\\
\le&~\nbr{\Sigmab_{k}^{-1}}_2\nbr{\Ub_{k}^\ts}_2\nbr{\Omegab}_2\nonumber\\
=&~\frac{1}{\sigma_k}\le~\frac{1}{\gamma}\label{eq:psth5_last}
\end{flalign}
In the first inequality, we have used submultiplicativity. Further,  next steps follow from  $\nbr{\Ub_{k}^\ts}_2=1$ and from Section~\ref{sec:notations}, it is easy to verify that
$
\Omegab^\ts\Omegab=\Ib_c~~\ie \nbr{\Omegab}_2=1\nonumber
$

The last step in eqn.~\eqref{eq:psth5_last} holds as $\sigma_i\ge\gamma$, ~ for all $i=1,\dots,k$

Finally, combining eqns.~\eqref{eq:psiter2},~\eqref{eq:psrecur71} and~\eqref{eq:psth5_last}, we conclude
\begin{flalign*}
\nbr{(\wb-\mb)^\ts(\widehat{\Fb} -\Fb)}_2\le\frac{\ve^t}{\gamma}~\nbr{\alphab_{k}}_2.
\end{flalign*}


==> Proof_of_sampling.tex <==
%!TEX root = arxiv_LDA.tex

\section{Proof of Theorem~\ref{thm:matmul}}\label{sxn:proof_sampling}
%
This result is similar in spirit to Theorem 4.2 of \citet{Holod15}, but our objective and (therefore) the analysis are slightly different in two ways. First, \cite{Holod15} presented a probabilistic bound for the 2-norm of the  relative error whereas our bound holds for the 2-norm of the absolute error. Second, we have an additional condition $\|\Zb\|_2\le 1$ which enables us to come up with a minimum value for $s$ that depends only on $\|\Zb\|_F^2$ and not on the stable rank of $\Zb$.

We first state two auxiliary results: a stable rank (intrinsic dimension) matrix Bernstein concentration inequality (Theorem~\ref{ineq:bern}) and a bound for the singular values of a difference of positive semi-definite matrices (Theorem~\ref{th:sing_diff}).
We then utilize these two results to obtain a proof of Theorem~\ref{thm:matmul}.

% \subsection{Auxiliary results}\label{sxn_F1}

\begin{theorem}\label{ineq:bern}\emph{(Theorem 7.3.1 of \cite{Tro15})}
	Let $\Yb_j$ be $s$ independent real symmetric random matrices, with $\EE(\Yb_j)=\mathbf{0}$~, $j=1,2,\dots ,s$. Let $\max_{1\le j\le s}\|\Yb_j\|_2\le\rho_1$ and $\Pb$ be a symmetric positive semi-definite matrix such that $\sum_{j=1}^s\EE(\Yb_j^2)\preccurlyeq\Pb$. Then, for any $\ve\ge\|\Pb\|_2^{1/2}+\rho_1/3$, we have
	\begin{flalign}
		\PP\left(\nbr{\sum_{j=1}^s\Yb_j}_2\ge\ve\right)\le 4\intdim(\Pb)\exp\left(-\frac{\ve^2/2}{\|\Pb\|_2+\rho_1\ve/3}\right)\nonumber
	\end{flalign}
	where $\intdim(\Pb)\defeq \tr(\Pb) / \|\Pb\|_2$.
\end{theorem}

\begin{theorem}\label{th:sing_diff}\emph{(Theorem 2.1 of \cite{Zhan01})}
	If $\Mb$ and $\Nb$ are real symmetric positive semi-definite matrices $\in\RR{m}{m}$, with singular values $\sigma_1(\Mb)\ge\sigma_2(\Mb)\ge\dots\ge\sigma_m(\Mb)$ and $\sigma_1(\Nb)\ge\sigma_2(\Nb)\ge\dots\ge\sigma_m(\Nb)$, then the singular values of the difference $\Mb - \Nb$ is bounded by
	$$\sigma_j(\Mb-\Nb)\le\sigma_j
	\begin{pmatrix}[c]
	\Mb & \mathbf{0}\\
	\mathbf{0} & \Nb
	\end{pmatrix},\qquad 1\le j\le m. $$
	In particular, we have $\|\Mb-\Nb\|_2\le\max\{\|\Mb\|_2,\|\Nb\|_2\}$.
\end{theorem}

% \subsection{Main proof}\label{sxn_F2}
%
\paragraph{Proof of Theorem~\ref{thm:matmul}.}
%
Let $\rank(\Zb)=\rho$ and $\Zb=\Ub_{\Zb}\Sigmab_{\Zb}\Vb_{\Zb}^\ts$ be the thin SVD representation of $\Zb$ with $\Ub_{\Zb}\in\RR{d}{\rho}$, $\Vb_{\Zb}\in\RR{n}{\rho}$ such that $\Ub_{\Zb}^\ts\Ub_{\Zb}=\Vb_{\Zb}^\ts\Vb_{\Zb}=\Ib_\rho$. Also, $\Sigmab_{\Zb}\in\RR{\rho}{\rho}$ is the diagonal matrix consisting of the non-zero singular values of $\Zb$ arranged in a non-increasing order $\ie$~$\sigma_1(\Zb)\ge\sigma_2(\Zb)\ge\dots\ge\sigma_\rho(\Zb)>0$.
Recall that we assume $\|\Zb\|_2=\sigma_1(\Zb)\le 1$.

Setting $\Cb=\Zb^\ts\Sb$, we have
\begin{flalign}
	\Zb^\ts\Sb\Sb^\ts\Zb-\Zb^\ts\Zb
	=&~\Cb\Cb^\ts-\Zb^\ts\Zb=\sum_{j=1}^s\Cb_{*j}(\Cb^\ts)_{j*}-\Zb^\ts\Zb
	% = \sum_{j=1}^s\left(\Cb_{*j}(\Cb^\ts)_{j*}-\frac{1}{s}\Zb^\ts\Zb\right)
	=\sum_{j=1}^s\Yb_j\label{eq:sampling_1}
\end{flalign}
where $\Yb_j=\Cb_{*j}(\Cb^\ts)_{j*}-\frac{1}{s}\Zb^\ts\Zb$.

Clearly,
\begin{flalign}
	\EE(\Yb_j)
	& = \EE\left(\Cb_{*j}(\Cb^\ts)_{j*}-\frac{1}{s}\Zb^\ts\Zb\right)=\EE\left(\Cb_{*j}(\Cb^\ts)_{j*}\right)-\frac{1}{s}\Zb^\ts\Zb\nonumber\\
	& = \sum_{i=1}^d\left(\frac{(\Zb^\ts)_{*i}}{\sqrt{sp_i}}\frac{\Zb_{i*}}{\sqrt{sp_i}}\right)p_i-\frac{1}{s}\Zb^\ts\Zb=\frac{1}{s}\sum_{i=1}^d(\Zb^\ts)_{*i}\Zb_{i*}-\frac{1}{s}\Zb^\ts\Zb\nonumber\\
	& = \frac{1}{s}\Zb^\ts\Zb-\frac{1}{s}\Zb^\ts\Zb=\mathbf{0},
\end{flalign}
where the third equality follows from Algorithm~2 and the definition of expectation. Thus, we have shown that $\Yb_j$'s have zero-mean. Next, we check that the assumptions of Theorem~\ref{ineq:bern} are satisfied.

\emph{Bound for $\max_{1\le j\le s}\|\Yb_j\|_2$.} As per eqn.~\eqref{eq:sampling_1}, $\Yb_j=\Cb_{*j}(\Cb^\ts)_{j*}-\frac{1}{s}\Zb^\ts\Zb$ is a difference of two positive semi-definite matrices. We apply Theorem~\ref{th:sing_diff} to obtain
\begin{flalign}
	\|\Yb_j\|_2=&~\nbr{\Cb_{*j}(\Cb^\ts)_{j*}-\frac{1}{s}\Zb^\ts\Zb}_2\le\max\left\{\nbr{\Cb_{*j}(\Cb^\ts)_{j*}}_2,\nbr{\frac{1}{s}\Zb^\ts\Zb}_2\right\}\nonumber\\[4pt]
	\le&~\max_{1\le i\le d}\left\{\nbr{\frac{(\Zb^\ts)_{*i}}{\sqrt{sp_i}}\frac{\Zb_{i*}}{\sqrt{sp_i}}}_2,\nbr{\frac{1}{s}\Zb^\ts\Zb}_2\right\}
	=~\frac{1}{s}\max_{1\le i\le d}\left\{\frac{\|\Zb_{i*}\|_2^2}{p_i},\|\Zb\|_2^2\right\}\nonumber\\[4pt]
	=&~\frac{1}{s}\max_{1\le i\le d}\left\{\frac{\|\Zb_{i*}\|_2^2}{\left(\|\Zb_{i*}\|_2^2/\|\Zb\|_F^2\right)},\|\Zb\|_2^2\right\}
	=~\frac{\|\Zb\|_F^2}{s}\label{eq:sampling_2}
\end{flalign}
which holds for all $j= 1,2,\dots s$.

Thus, we have shown that $\max_{1\le j\le s}\|\Yb_j\|_2\le\frac{\|\Zb\|_F^2}{s} \defeq \rho_1$.

\bigskip
\emph{The matrix $\Pb$.} From the definition of $\Yb_j$ in eqn.~\eqref{eq:sampling_1}, we have
\begin{flalign}
	& \Yb_j=\Cb_{*j}(\Cb^\ts)_{j*}-\frac{1}{s}\Zb^\ts\Zb \\
	\Rightarrow \ &  \Yb_j+\frac{1}{s}\Zb^\ts\Zb=\Cb_{*j}(\Cb^\ts)_{j*}\nonumber\\
	\Rightarrow \ & \left(\Yb_j+\frac{1}{s}\Zb^\ts\Zb\right)^2
	= \left(\Cb_{*j}(\Cb^\ts)_{j*}\right)^2=\Cb_{*j}(\Cb^\ts)_{j*}\Cb_{*j}(\Cb^\ts)_{j*}\nonumber\\
	\Rightarrow \ & \Yb_j^2-\Yb_j\Zb^\ts\Zb-\Zb^\ts\Zb\Yb_j+\frac{1}{s^2}(\Zb^\ts\Zb)^2
	=\Cb_{*j}(\Cb^\ts)_{j*}\Cb_{*j}(\Cb^\ts)_{j*}.
	\label{eq:sampling_3}
\end{flalign}
%
Taking expectations on both sides of eqn.~\eqref{eq:sampling_3} and noting that $\EE(\Yb_j)=\mathbf{0}$ gives
\begin{flalign}
	\EE(\Yb_j^2)+\frac{1}{s^2}(\Zb^\ts\Zb)^2
	& = \EE(\Cb_{*j}(\Cb^\ts)_{j*}\Cb_{*j}(\Cb^\ts)_{j*})\nonumber\\
	& = \sum_{i=1}^d\left(\frac{(\Zb^\ts)_{*i}}{\sqrt{sp_i}}\frac{\Zb_{i*}}{\sqrt{sp_i}}\frac{(\Zb^\ts)_{*i}}{\sqrt{sp_i}}\frac{\Zb_{i*}}{\sqrt{sp_i}}\right)p_i\nonumber\\
	& = \frac{1}{s^2}\sum_{i=1}^d(\Zb^\ts)_{*i}\left(\frac{\|\Zb_{i*}\|_2^2}{p_i}\right)\Zb_{i*}=\frac{1}{s^2}\sum_{i=1}^d\left(\frac{\|\Zb_{i*}\|_2^2}{\|\Zb_{i*}\|_2^2/\|\Zb\|_F^2}\right)(\Zb^\ts)_{*i}\Zb_{i*}\nonumber\\
	& = \frac{\|\Zb\|_F^2}{s^2}\sum_{i=1}^d(\Zb^\ts)_{*i}\Zb_{i*}=\frac{\|\Zb\|_F^2}{s^2}\Zb^\ts\Zb.
	\label{eq:sampling_4}
\end{flalign}
%
Summing both sides of eqn.~\eqref{eq:sampling_4} over $j$ gives
\begin{flalign}
	\sum_{j=1}^s\EE(\Yb_j^2)&=~\frac{\|\Zb\|_F^2}{s}\Zb^\ts\Zb-\frac{1}{s}(\Zb^\ts\Zb)^2\nonumber\\
	&\preccurlyeq~\frac{\|\Zb\|_F^2}{s}\Zb^\ts\Zb=\frac{\|\Zb\|_F^2}{s}\Vb_{\Zb}\Sigmab_{\Zb}^2\Vb_{\Zb}^\ts\nonumber\\
	&\preccurlyeq~\frac{\|\Zb\|_F^2}{s}\Vb_{\Zb}\Db\Vb_{\Zb}^\ts\defeq \Pb ,
	\label{eq:sampling_7}
\end{flalign}
where $\Db\in\RR{\rho}{\rho}$ is diagonal matrix whose $i$-th diagonal entry is equal to
$$
\Db_{ii} = \left\{
\begin{array}{ll}
1 & \text{if}\quad i=1 \\
\sigma_i^2(\Zb) & \text{otherwise}.
\end{array}
\right.
$$
%
The second-to-last inequality in eqn.~\eqref{eq:sampling_7} holds because $\sum_{j=1}^s\EE(\Yb_j^2)$, $\frac{\|\Zb\|_F^2}{s}\Zb^\ts\Zb$ and $\frac{1}{s}(\Zb^\ts\Zb)^2$ are all positive semi-definite matrices. Further, the last inequality follows from the fact $\Sigmab_{\Zb}^2\preccurlyeq\Db$ as $\sigma_1(\Zb)=\|\Zb\|_2\le1$. 

Note that $\|\Db\|_2=1$ and
\begin{flalign}
	\Tr{\Db}=&~1+\sum_{i=2}^\rho\sigma_i^2(\Zb)=1-\sigma_1^2(\Zb)+\sum_{i=1}^\rho\sigma_i^2(\Zb)\nonumber\\
	=&~1-\sigma_1^2(\Zb)+\|\Zb\|_F^2\le~1+\|\Zb\|_F^2.\label{eq:trD}
\end{flalign}
%
Again,
\begin{flalign}
	\|\Pb\|_2=\frac{\|\Zb\|_F^2}{s}\nbr{\Vb_{\Zb}\Db\Vb_{\Zb}^\ts}_2=\frac{\|\Zb\|_F^2}{s}\nbr{\Db}_2=\frac{\|\Zb\|_F^2}{s}\label{eq:P_2}
\end{flalign}
where the second equality follows from the unitary invariance of 2-norm.
%
Similarly, from eqn.~\eqref{eq:trD}
\begin{flalign}
	\Tr{\Pb}=\frac{\|\Zb\|_F^2}{s}\Tr{\Vb_{\Zb}\Db\Vb_{\Zb}^\ts}=\frac{\|\Zb\|_F^2}{s}\Tr{\Db}\le\frac{\|\Zb\|_F^2}{s}(1+\|\Zb\|_F^2)\label{eq:tr_P}
\end{flalign}
%
Combining eqns.~\eqref{eq:P_2} and \eqref{eq:tr_P} yields
\begin{flalign}
	\intdim(\Pb)=\frac{\Tr{\Pb}}{\|\Pb\|_2}\le \frac{\frac{\|\Zb\|_F^2}{s}(1+\|\Zb\|_F^2)}{\frac{\|\Zb\|_F^2}{s}}=1+\|\Zb\|_F^2.
\end{flalign}


\emph{Application of Theorem~\ref{ineq:bern}.}
%
From eqn.~\eqref{eq:sampling_1}, we have
\begin{flalign}
	\PP\left(\nbr{\Zb^\ts\Sb\Sb^\ts\Zb-\Zb^\ts\Zb}_2>\ve\right)
	=\PP\left(\nbr{\sum_{j=1}^s\Yb_j}_2>\ve\right). \label{eq:PP}
\end{flalign}
%
Applying Theorem~\ref{ineq:bern} to the right hand side of eqn.~\eqref{eq:PP} yields:
\begin{flalign}
	\PP\left(\nbr{\sum_{j=1}^s\Yb_j}_2>\ve\right)\le&~4\intdim(\Pb)\exp\left(-\frac{\ve^2/2}{\|\Pb\|_2+\rho_1\ve/3}\right)\nonumber\\
	\le&~4(1+\|\Zb\|_F^2)\exp\left(-\frac{\ve^2/2}{\frac{\|\Zb\|_F^2}{s}+ \frac{\ve\|\Zb\|_F^2}{3s}}\right)\nonumber\\
	=&~4(1+\|\Zb\|_F^2)\exp\left(-\frac{s\ve^2}{\|\Zb\|_F^2\left(2+2\ve/3\right)}\right). \label{eq:sampling_6}
\end{flalign}
%
Clearly, $\PP\left(\nbr{\Zb^\ts\Sb\Sb^\ts\Zb-\Zb^\ts\Zb}_2>\ve\right)\le\delta$ holds if the right hand side of eqn.~\eqref{eq:sampling_6} is at most $\delta$, \ie,
\begin{flalign}
	4(1+\|\Zb\|_F^2)\exp\left(-\frac{s\ve^2}{\|\Zb\|_F^2\left(2+2\ve/3\right)}\right)\le~\delta
	\iff&\frac{s\ve^2}{\|\Zb\|_F^2\left(2+2\ve/3\right)}\ge\ln\left(\frac{4(1+\|\Zb\|_F^2)}{\delta}\right)\nonumber\\[4pt]
	\iff& s\ge\left(2+\frac{2\ve}{3}\right)~\frac{\|\Zb\|_F^2}{\ve^2}~\ln\left(\frac{4(1+\|\Zb\|_F^2)}{\delta}\right). \label{eq:pr2}
\end{flalign}
%
As $\ve\le 1$, eqn.~\eqref{eq:pr2} holds if
$$s\ge~\frac{8\|\Zb\|_F^2}{3~\ve^2}~\ln\left(\frac{4(1+\|\Zb\|_F^2)}{\delta}\right).$$
% which proves the theorem.

Finally, it still remains to be shown that the last condition of Theorem~\ref{ineq:bern} is satisfied, \ie, $\ve\ge\|\Pb\|_2^{1/2}+\rho_1/3$. We solve the following equation for $\ve$:
\begin{flalign}
	& 4\big(1+\|\Zb\|_F^2\big)\exp\left(-\frac{s\ve^2}{\|\Zb\|_F^2\left(2+2\ve/3\right)}\right)=\delta\nonumber\\[4pt]
	\implies&~ 3s\ve{^2}-2\|\Zb\|_F^2\ln\left(\frac{4(1+\|\Zb\|_F^2)}{\delta}\right)\ve-6\|\Zb\|_F^2\ln\left(\frac{4(1+\|\Zb\|_F^2)}{\delta}\right)=0\nonumber\\[4pt]
	\implies&~\ve=\beta+\sqrt{\beta^2+6\beta} , \nonumber
\end{flalign}
where
\[
\beta=\frac{\|\Zb\|_F^2\ln\left(\frac{4(1+\|\Zb\|_F^2)}{\delta}\right)}{3s} \,.
\]
Observe that, $\ve\ge\frac{\rho_1}{3}+\|\Pb\|_2^{1/2}$ if $\beta\ge\frac{\rho_1}{3}$ and $6\beta\ge\|\Pb\|_2$.
Both conditions will be satisfied if
\[
\ln\left(\frac{4(1+\|\Zb\|_F^2)}{\delta}\right)\ge 1
\iff \delta\le\frac{4(1+\|\Zb\|_F^2)}{e}
\]
which is always true since $\delta<1$. This concludes the proof.
\qed
%

